Belief Revision, Minimal Change and Relaxation: A General Framework based on Satisfaction Systems, and Applications to Description Logics

Belief revision of knowledge bases represented by a set of sentences in a given logic has been extensively studied but for specific logics, mainly propositional, and also recently Horn and description logics. Here, we propose to generalize this operation from a model-theoretic point of view, by defining revision in an abstract model theory known under the name of satisfaction systems. In this framework, we generalize to any satisfaction systems the characterization of the well known AGM postulates given by Katsuno and Mendelzon for propositional logic in terms of minimal change among interpretations. Moreover, we study how to define revision, satisfying the AGM postulates, from relaxation notions that have been first introduced in description logics to define dissimilarity measures between concepts, and the consequence of which is to relax the set of models of the old belief until it becomes consistent with the new pieces of knowledge. We show how the proposed general framework can be instantiated in different logics such as propositional, first-order, description and Horn logics. In particular for description logics, we introduce several concrete relaxation operators tailored for the description logic $\ALC{}$ and its fragments $\EL{}$ and $\ELext{}$, discuss their properties and provide some illustrative examples.

==> Arts.tex <==
In the last decade, several works have studied revision operators in Description Logics. While most of them concentrated on the adaptation of AGM theory, few works have addressed  the definition of concrete operators~\cite{meyer2005knowledge,qi2006revision,QLB06}. A closely related field is inconsistency handling in ontologies (e.g.~\cite{schlobach2003non,schlobach2007debugging}), with the main difference that the rationality of inconsistency  repairing operators is not investigated, as suggested by AGM theory.

Some of our relaxation operators are closely related to the ones introduced in~\cite{QLB06} for knowledge bases revision and in~\cite{Gorogiannis2008a} for merging first-order theories. Our relaxation-based revision framework, being abstract enough (i.e. defined through easily satisfied properties), encompasses these operators.  Moreover,  the revision operator defined in~\cite{QLB06} considers only  inconsistencies due to Abox assertions. Our operators are general in the sense that Abox assertions are handled as any formula of the language. 

 The relaxation idea originates from the work on Morpho-Logics, initially introduced in~\cite{BL02,BPU04}. In this seminal work, revision operators (and explanatory relations) were defined through dilation and erosion operators. These operators share some similarities with relaxation and retraction as defined in this paper. Dilation is a sup-preserving operator and erosion is inf-preserving, hence both are increasing. Some particular dilations and erosions are exhaustive and extensive while relaxation and retraction operators are defined to be exhaustive and extensive but not necessarily sup- and inf-preserving. 
 
\Isa{Ce paragraphe est-il vraiment \`a enlever ? passe dans la conclusion ?} Another contribution in this paper concerns the generalization of AGM postulates and their translation in a model-theoretic writing with a  definition of inconsistency, allowing using them in a wide class of non-classical logics. This follows recent  works on the adaptation of AGM theory (e.g.~\cite{DP15,flouris2005applying,RW14,RWFA13}). Our generalization is closely related to the one recently introduced in~\cite{RW14} and could be seen as its counterpart in a model-theoretic setting. It also extends the one introduced in~\cite{QLB06}.


==> DL_Introduction.tex <==
%\del{Belief revision is at the core of artificial intelligence and philosophy questionings. It is defined as the process of changing an agent belief with a new acquired  knowledge. Three change operations are usually considered: {\em  expansion, contraction} and {\em revision}. 
%Belief expansion refers to the process of adding the  agent's belief with a new acquired one without checking inconsistency, contraction is the process of removing a set of beliefs from the old agent's ones, and revision refers 
%We focus here on the revision, i.e. the process of adding {\bf consistently} the new belief sets. 
%Belief revision has been intensively studied in classical logics (e.g. propositional logic) mostly under the prism of AGM theory~\cite{AGM-85}. With the growing interest in non-classical logics, such as Horn Logics and Description Logics~\cite{Baad03nocrossref}, several attempts to generalize AGM theory, making it compliant to the meta-logical flavor of these logics, have been introduced recently~\cite{flouris2005applying,delgrande2015,ribeiro2013,ribeiro2014}.  }
%
%In~\cite{ARXIV}, we introduced a general framework for belief revision in arbitrary logics, based both on the theory of institutions~\cite{Dia08,GB92} and on relaxations~\cite{FD:KR-14}. In this part, we consider the case of Description Logics (DLs), as particular institutions, and introduce concrete relaxation operators for different fragments of the DL $\ALC{}$. 

Description Logics  are now pervasive in many knowledge-based representation systems, such as ontological reasoning, semantic web, scene understanding, cognitive robotics, to mention a few. In all these domains, the expert knowledge is not fixed, but rather a flux evolving over time, hence requiring  the definition of rational revision operators. Revision is then a cornerstone in ontology engineering life-cycle where the expert knowledge is prone to change and inconsistency. 

Due to this growing interest in DLs,  several attempts to generalize the well-known AGM theory, making it compliant with the meta-logical flavor of these logics, have been introduced recently~\cite{delgrande2015,flouris2005applying,ribeiro2014,ribeiro2013}. Indeed, AGM theory in its original form defines a set of rational postulates requiring the logic to be closed under usual propositional connectives $(\vee, \wedge, \implies, \neg)$ which prevents its use in many non-classical logics, including DLs.  Indeed, many DLs do not allow for negation of concepts (e.g. $\EL{}$) and a fortiori disjunction between TBox and ABox sentences is not defined in all DLs.   Recently, many papers have addressed the adaptation of AGM theory to non-classical logics, e.g.~\cite{delgrande2015,flouris2005applying,ribeiro2014,ribeiro2013}. The first efforts concentrated on the adaptation of contraction postulates, but more recently, the adaptation of revision postulates and the introduction of new minimality criteria were also addressed~\cite{ribeiro2014}, not necessarily related to the contraction  operator, throwing out the need for negation. One can find in~\cite{qi2006} an attempt to adapt the AGM revision postulates to DL in a model-theoretic way, following the seminal work of~\cite{KatsunoMendelzon91} that translated the AGM postulates in propositional logic semantics. 

In this paper, we follow an alternative path by instantiating our abstract framework. Indeed,  the AGM postulates are generalized from a model-theoretic standpoint, allowing  widening their scope to a more general family of logics, including Description Logics.% A key point in this generalization is to translate AGM postulates  in a categorical abstract model theory, the theory of institutions, which formalizes the intuitive notion of a logical system, including syntax, semantics and satisfaction relation. In this abstract framework, revision has been directly defined instead of indirectly through the Levi identity from expansion and contraction which requires the underlying logic to be equipped with negation. 
%Besides, the notion of  negation is defined  in a general way, which allows  defining directly the revision operator instead of indirectly defining it through the Levi identity from the contraction as classically done.

Hence, this paper contributes to the effort of defining such  rational revision operators, in line with the recent work in this domain~\cite{flouris2006inconsistencies,flouris2005applying,qi2006revision,qi2006}. 
%This paper is organized as follows. 
%Section~\ref{sec:Preliminaries} 
%recalls  some  definitions  about Description Logics and summarizes  our contribution in~\cite{ARXIV}. Our main contribution is detailed in Section~\ref{sec:concrete}, by providing concrete theory relaxation operators in different DLs (namely $\ALC{}$ and its fragments $\EL{}$ and $\ELext{}$). Section~\ref{sec:related} positions our contributions with regards to the literature, and finally Section~\ref{sec:conc} draws some conclusions and perspectives. 



%Belief revision: Let $T$ and $T'$ be two knowledge bases, belief revision refers to the process of adding consistently the new piece of knowledge $T'$ to the old knowledge $T$. 
\fbox{Needs for adaptation in what follows!}

The paper is organized as follows. Section~\ref{institutions} reviews some concepts, notations and terminology about \Marc{satisfaction systems} which are used in this work. In Section~\ref{AGM postulates for revision}, we adapt AGM theory in the framework of \Marc{satisfaction systems}, and then give an abstract model-theoretic rewriting of AGM postulates. We then show in Section~\ref{Orders and AGM postulates} that any revision operator satisfying such postulates accomplishes an update with minimal change to the set of models of knowledge bases. In Section~\ref{Relaxation and AGM postulates}, we introduce a general framework of relaxation-based revision operators and show that our revision operators lead to faithful assignments and then satisfy AGM postulates. In Section~\ref{applications}, we illustrate our abstract approach by providing revision operators in different logics, including classical logics (propositional and first order logics) and non-classical ones (Horn and description logics). Finally, Section~\ref{related works} is dedicated to related works. 



==> Reserve.tex <==
In Theorem~\ref{correspondence agm and orders}, we showed for every revision operator $\circ$ that satisfies Postulates (G1)-(G6), that there exists a binary relation over models $\preceq_T$ which is faithful and meets all the conditions of Theorem~\ref{correspondence agm and orders}. Here, we define a binary relation on models that we will also note  $\preceq_T$, that only works (i.e. satisfies all the properties of Theorem~\ref{correspondence agm and orders}) for revision operators based on relaxations.

\medskip
Given $T,T' \subseteq Sen(\Sigma)$, let us start by defining $\preceq^{T'}_T \subseteq Mod(T') \times Mod(T')$ as follows:

$$\mathcal{M} \preceq^{T'}_T \mathcal{M}' \Longleftrightarrow \mathcal{M} \in Mod(T \circ T') \wedge \mathcal{M}' {\not \in} Mod(T \circ T')$$

Let us set $\preceq_T = \bigcup_{T'} \preceq^{T'}_T$.~\footnote{Let us note that $\preceq_T \subseteq Mod(\Sigma) \times Mod(\Sigma)$ because $\preceq^\emptyset_T \subseteq \preceq_T$.} 

\begin{theorem}
\label{is a FA}
$\preceq_T$ is faithful. Moreover, for every knowledge base $T' \subseteq Sen(\Sigma)$:

\begin{itemize}
\item if $T'$ is consistent, then $Min(Mod(T') \setminus Triv,\preceq_T) \neq \emptyset$.
\item $Mod(T \circ T') \setminus Triv  = Min(Mod(T') \setminus Triv,\preceq_T)$. 
\item For every $T'' \subseteq Sen(\Sigma)$, if $(T \circ T') \cup T''$ is consistent, then $Min(Mod(T') \setminus Triv,\preceq_T) \cap Mod(T'') = Min(Mod(T' \cup T'') \setminus Triv,\preceq_T)$.
\end{itemize}
\end{theorem}

\begin{proof}
Let us first show that $\preceq_T$ is faithful. Obviously, we have for every $\mathcal{M},\mathcal{M}' \in Mod(T)$ and every $T' \subseteq Sen(\Sigma)$ that both $\mathcal{M} {\not \preceq^{T'}_T} \mathcal{M}'$ and $\mathcal{M}' {\not \preceq^{T'}_T} \mathcal{M}$. \\ Let $\mathcal{M} \in Mod(T)$ and let $\mathcal{M}' \in Mod(\Sigma) \setminus Mod(T)$. Obviously, we have that $\mathcal{M} \preceq^\emptyset_T \mathcal{M}'$. Let $T' \subseteq Sen(\Sigma)$ such that $\mathcal{M},\mathcal{M}' \in Mod(T')$. By defintion of $\circ$, we have that $\mathcal{M} \in Mod(T \circ  T')$ but $\mathcal{M}' {\not \in} Mod(T \circ T')$ , and then $\mathcal{M}' {\not \preceq^{T'}_T} \mathcal{M}$. \\
Let us prove that $Mod(T \circ T') \setminus Triv = Min(Mod(T') \setminus Triv,\preceq_T)$. This will directly prove that $Min(Mod(T') \setminus Triv,\preceq_T) \neq \emptyset$ when $T'$ is consistent. Indeed, by definition, we have that $T \circ T'$ is consistent when $T'$ is consistent, and then $Min(Mod(T') \setminus Triv,\preceq_T)  \neq \emptyset$ if $Mod(T \circ T') \setminus Triv = Min(Mod(T') \setminus Triv,\preceq_T)$. \\
If $T'$ is inconsistent, then so is $T \circ T'$ by definition. Hence, $Mod(T \circ T') \setminus Triv = Min(Mod(T') \setminus Triv,\preceq_T) = \emptyset$. Let us suppose that $T'$ is consistent.
\begin{itemize}
\item $Mod(T \circ T') \setminus Triv  \subseteq Min(Mod(T') \setminus Triv,\preceq_T)$. Let $\mathcal{M} \in Mod(T \circ T') \setminus Triv$. Let $\mathcal{M}' \in Mod(T') \setminus Triv$. Two cases have to be considered:

\begin{enumerate}
\item $\mathcal{M}' \in Mod(T \circ T')$. Obviously, we have that both $\mathcal{M} {\not \preceq^{T'}_T} \mathcal{M}'$ and $\mathcal{M}' {\not \preceq^{T'}_T} \mathcal{M}$. Let us show that this is also true for every $T'' \subseteq Sen(\Sigma)$ such that $\mathcal{M},\mathcal{M}' \in Mod(T'')$. By hypothesis, we then have that $\mathcal{M},\mathcal{M}' \in Mod((T \circ T') \cup T'')$, and then $(T \circ T') \cup T''$ is consistent. By Conditions 2. and 3. of Defintion~\ref{revision based in relaxation}, we then have that $(T \circ T') \cup T'' = T \circ (T' \cup T'')$. Now, we obviously have that $T'' \leq_T T' \cup T''$. Therefore, if $T \circ T' = \rho^\mathcal{K}(T) \cup T'$ and $T \circ T'' = \rho^{\mathcal{K}'}(T) \cup T'$, then by Condition 3. of Defintion~\ref{revision based in relaxation}, for every $\varphi \in T$, we have that $k'_\varphi \leq k_\varphi$. Here, we have also to consider two cases:

\begin{enumerate}
\item $\mathcal{M} \in Mod(T \circ T'')$ or $\mathcal{M}' \in Mod(T \circ T'')$. Let us suppose that $\mathcal{M} \in Mod(T \circ T'')$ (the conclusion is similar if we choose $\mathcal{M}' \in Mod(T \circ T'')$). In this case, by Condition 2. of Defintion~\ref{revision based in relaxation}, we have that $\sum \mathcal{K} \leq \sum \mathcal{K'}$, and then $\mathcal{K} = \mathcal{K}'$. Hence, we can deduce that $\mathcal{M}' \in Mod(T \circ T'')$, and then $\mathcal{M} {\not \preceq^{T''}_T} \mathcal{M}'$ and $\mathcal{M}' {\not \preceq^{T''}_T} \mathcal{M}$.
\item $\mathcal{M},\mathcal{M}' {\not \in} Mod(T \circ T'')$. We then have by definition that both $\mathcal{M} {\not \preceq^{T''}_T} \mathcal{M}'$ and $\mathcal{M}' {\not \preceq^{T''}_T} \mathcal{M}$.
\end{enumerate}
\item $\mathcal{M}' {\not \in} Mod(T \circ T')$. By definition of $\preceq^{T'}_T$, we have that $\mathcal{M} \preceq^{T'}_T \mathcal{M}'$. 
\end{enumerate}
 
\item $Min(Mod(T') \setminus Triv,\preceq_T) \subseteq Mod(T \circ T') \setminus Triv$. Let $\mathcal{M} \in Min(Mod(T') \setminus Triv,\preceq_T)$. Let us suppose that $\mathcal{M} {\not \in} Mod(T \circ T') \setminus Triv$. As $T'$ is consistent, then so is $T \circ T'$. Hence, there exists $\mathcal{M}' \in Mod(T \circ T') \setminus Triv$. As $\mathcal{M} \in Mod(T')$, we have that $\mathcal{M}' \preceq^{T'}_T \mathcal{M}$, and then so is $\mathcal{M} \preceq_T \mathcal{M}'$. This means there exists $T'' \subseteq Sen(\Sigma)$ such that $\mathcal{M},\mathcal{M}' \in Mod(T'')$, $\mathcal{M} \in Mod(T \circ T'')$ and $\mathcal{M}' {\not \in} Mod(T \circ T'')$. By hypothesis, we have both that $(T \circ T') \cup T''$ and $(T \circ T'') \cup T'$ are consistent. Therefore, by Conditions 2. and 3. of Definition~\ref{revision based in relaxation}, we have that $(T \circ T') \cup T'' = (T \circ T'') \cup T'$, and then $\mathcal{M} \in Mod(T \circ T') \setminus Triv$ and $\mathcal{M}' \in Mod(T \circ T'') \setminus Triv$, which are contradictions.  
\end{itemize}
Finally, to prove the last point, we follow the same step than in the proof of Theorem~\ref{correspondence agm and orders}. 
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%

in~\cite{RW14} in addition to the standard AGM postulates for revision, the authors to express their minimality criteria on removed formul\ae~ introduced the postulate (Relevance) that can be written in our framework as follows:

\begin{center}
{\bf (Relevance)} if $\varphi \in T \setminus (T \circ T')$, then there exists $X$, $T \cap (T \circ T') \subseteq X \subseteq T$, such that $Cn(X \cup T') \neq Sen(\Sigma)$ and $Cn(X \cup \{\varphi\} \cup T') = Sen(\Sigma)$
\end{center}  

And, we have the following result.

\begin{proposition}
The revision operator of Definition~\ref{revision based in relaxation} satisfies (Relevance).
\end{proposition}

\begin{proof}
Let $\varphi \in T_1 \setminus (T_1 \circ T_2)$. By definition, this means that $\varphi \in T'_1$ where $T'_1 = \{\varphi \in T_1 \mid k_\varphi \neq 0\}$. Therefore, it is sufficient to set $X =  \{\varphi \in T_1 \mid k_\varphi = 0\}$. By Lemma~\ref{mimimality lemma}, the minimality criteria on removed formul\ae~of (Relevance) is obviously satisfied.
\end{proof}

%%%%%%%%%%%%%%%%%%%

The revision operators based on relaxations defined in Definition~\ref{revision based in relaxation} ensure minimality criteria on transformed formulas. 

\Marc{Le r\'esultat ci-dessous n'est vrai que si $T$ est consistante. Je pense que le r\'esultat n'est pas vrai en g\'en\'eral quand $T$ n'est pas consistante.}

\begin{proposition}
\label{mimimality lemma}
From the revision operator $\circ$ defined in Definition~\ref{revision based in relaxation}, for every $T,T' \subseteq Sen(\Sigma)$ such that $T$ and $T'$ are consistent, we have: If $T \circ T' = \rho^\mathcal{K}(T) \cup T'$, then by denoting $T_1 = \{\varphi \in T \mid k_\varphi \neq 0\}$ and $T_2 = T \setminus T_1$

$$\forall T''~\mbox{s.t.}~ T_2 \subset T'' \subseteq T, Cn(T' \cup T'') = Sen(\Sigma)$$
\end{proposition}

\begin{proof}
The property directly results from: 

$$\forall \varphi \in T_1, Cn(T' \cup T_2 \cup \{\varphi\}) = Sen(\Sigma)$$ 

\noindent
Let suppose the contrary, i.e., there exists $\varphi \in T_1$ such that $Cn(T' \cup T_2 \cup \{\varphi\}) \neq Sen(\Sigma)$. As $T$ is consistent and by the extensively condition, this means that for $\mathcal{K}' = (\mathcal{K} \setminus \{k_\varphi\}) \cup \{k_\varphi = 0\}$ we have $\rho^{\mathcal{K}'}(T) \cup T'$ is consistent. But, we have that $\sum \mathcal{K}' < \sum \mathcal{K}$, which contradicts the second condition of Defintion~\ref{revision based in relaxation}.  
\end{proof}


%%%%%%%%%%%%%%%%

As discussed in Section~\ref{applications}, relaxations can be directly about formulas without immediate expectation on models, and then be strongly dependent of syntax (see the case of revision in {\bf FOL} in Section~\ref{revision in FOL}). This then prevents to satisfy Postulate (G4) without an additional condition. The condition that we propose to satisfy Postulate (G4) is the following:

\begin{itemize}
\item[(A)] $\forall T,T' \subseteq Sen(\Sigma), Mod(T) = Mod(T')$ \\
\mbox{} \hfill $\Rightarrow (\forall \mathcal{K}_T, \exists \mathcal{K}_{T'}, Mod(\rho^{\mathcal{K}_T}(T)) = Mod(\rho^{\mathcal{K}_{T'}}(T')))$
\end{itemize}

In Section~\ref{applications}, we will give for each example application, either a proof that Condition (A) is satisfied, or a counter-example. 

\begin{theorem}
Condition (A) implies Postulate (G4). 
\end{theorem}

\begin{proof}
Let us suppose that $Cn(T_1) = Cn(T'_1)$ and $Cn(T_2) = Cn(T'_2)$. The case where $T_2$ (and then $T'_2$) is inconsistent is obvious. Then, let us suppose that $T_2$ and $T'_2$ are consistent. By definition of revision, we have:

\begin{center}
$T_1 \circ T_2 = \rho^\mathcal{K}(T_1) \cup T_2$ \\
$T'_1 \circ T'_2 = \rho^{\mathcal{K}'}(T'_1) \cup T'_2$
\end{center}
By Condition (A), we respectively have:

\begin{center}
$\exists \mathcal{K}'_1, Mod(\rho^\mathcal{K}(T_1)) = Mod(\rho^{\mathcal{K}'_1}(T'_1))$ \\
$\exists \mathcal{K}_1, Mod(\rho^{\mathcal{K}'}(T'_1)) = Mod(\rho^{\mathcal{K}_1}(T_1))$
\end{center} 
By the fact that $Cn(T_2) = Cn(T'_2)$, we have both that $\rho^{\mathcal{K}_1}(T_1) \cup T_2$  and $\rho^{\mathcal{K}'_1}(T'_1) \cup T'_2$ are consistent. By the minimality condition on $\mathcal{K}$ and $\mathcal{K}'$ and extensivity of relaxations, we have $Mod(\rho^\mathcal{K}(T_1)) \subseteq Mod(\rho^{\mathcal{K}_1}(T_1))$ and $Mod(\rho^{\mathcal{K}'}(T'_1)) \subseteq Mod(\rho^{\mathcal{K}'_1}(T'_1))$, whence by using both equations just above, we conclude that $Mod(\rho^\mathcal{K}(T_1)) = Mod(\rho^{\mathcal{K}_1}(T_1))$ and $Mod(\rho^{\mathcal{K}'}(T'_1)) = Mod(\rho^{\mathcal{K}'_1}(T'_1))$, and then $Mod(\rho^\mathcal{K}(T_1)) = Mod(\rho^{\mathcal{K}'}(T'_1))$. 
\end{proof}

\Marc{J'aimerais bien trouver un contre-exemple \`a la condition (A) dans {\bf FOL} ou {\bf DL}. Je cherche de mon cot\'e. Si vous avez des id\'ees de votre cot\'e.}

\Marc{L\`a, j'ai un probl\`eme avec la d\'efinition de $\preceq_T$ dans le th\'eor\`eme ci-dessous. En effet, pour d\'emontrer que $Min(Mod(T') \setminus Triv,\preceq_T) \neq \emptyset$ on a besoin d'imposer que $T$ est de cardinalit\'e finie. Qu'en pensez-vous ?}

What brought us to Condition (A) is the following result:

\begin{theorem}
\label{orders and relaxation}
From any $\Sigma$-relaxation $\rho$ we define for every \Marc{finite} knowledge base $T \subseteq Sen(\Sigma)$ the binary relation $\preceq_T \subseteq Mod(\Sigma) \times Mod(\Sigma)$ as follows: 

\medskip
\noindent
$\mathcal{M} \preceq_T \mathcal{M}'$ \\
\mbox{} \hfill $\Longrightarrow (\forall \mathcal{K}_T, \mathcal{M}' \in Mod(\rho^{\mathcal{K}_T}(T)) \Longrightarrow \mathcal{M} \in Mod(\rho^{\mathcal{K}_T}(T)))$

\medskip
\noindent
Then, $\preceq_T$  satisfies the first two conditions of Defintion~\ref{faithful assignment} and the third one if $\rho$ satisfies Condition (A). Moreover,  for every $T' \subseteq Sen(\Sigma)$, we have:

\begin{itemize}
\item if $T'$ is consistent, then $Min(Mod(T') \setminus Triv,\preceq_T) \neq \emptyset$.
\item $Mod(T \circ T') = Min(Mod(T') \setminus Triv,\preceq_T)$. 
\end{itemize}
\end{theorem}

\begin{proof}

%\Isa{Mais ce n'est plus tout \`a fait cela qu'il faut montrer...}

%Minimal elements are all models of $Mod(\rho^{\mathcal{K}_T}(T))$ such that $\mathcal{K}_T$ is the set containing the least natural numbers $k_\varphi$ such that $\rho^{\mathcal{K}_T}(T)$ is consistent (by exhaustivity, such a set exists). 

The first condition of FA is obvious by construction. Let $\mathcal{M} \in Mod(T)$ and $\mathcal{M}' \in Mod(\Sigma) \setminus Mod(T)$. By definition, for every $n \in \mathbb{N}$, $\mathcal{M} \in Mod(\rho^n(T))$. Moreover, by both conditions of relaxations, there exists $k \in \mathbb{N}$ such that $\mathcal{M}' \in Mod(\rho^k(T))$ and for every $k'$, $0 \leq k' < k$, $\mathcal{M}' {\not \in} Mod(\rho^{k'}(T))$. Hence, $\mathcal{M}' {\not \preceq}_T \mathcal{M}$. \\
To prove the third property of FA, let us suppose that $Mod(T) = Mod(T')$, and let us show that $\preceq_T = \preceq_{T'}$ under the hypothesis of Condition (A). Let $\mathcal{M} \preceq_T \mathcal{M}'$. Let $\mathcal{K}_{T'}$ such that $\mathcal{M}' \in Mod(\rho^{\mathcal{K}_{T'}}(T'))$. By Condition (A), there exists $\mathcal{K}_T$ such that $Mod(\rho^{\mathcal{K}_{T'}}(T')) = Mod(\rho^{\mathcal{K}_{T}}(T))$. Hence, $\mathcal{M}' \in Mod(\rho^{\mathcal{K}_{T}}(T))$, and then $\mathcal{M} \in Mod(\rho^{\mathcal{K}_{T}}(T))$ whence, we can conclude that $\mathcal{M}' \preceq_{T'} \mathcal{M}$. We can apply the same process to show that $\preceq_{T'} \subseteq \preceq_T$.\\ 
By construction, $\preceq_T$ is obviously a pre-order. Moreover, it is well-foundness. Indeed, let us suppose an infinite strictly decreasing sequence $(\mathcal{M}_i)_{i \in \mathbb{N}}$. By definition of $\preceq_T$, for every $i \in \mathbb{N}$, $\mathcal{M}_i \in Mod(\rho^{\mathcal{K}_T}(T)) \Rightarrow \mathcal{M}_{i+1} \in  Mod(\rho^{\mathcal{K}_T}(T))$. Let us note $\mathcal{K}$ the least set $\mathcal{K}_T$ such that $\mathcal{M}_0, \mathcal{M}_1 \in Mod(\rho^{\mathcal{K}_T}(T))$ (i.e. for every $\mathcal{K}'_T$ such that $\mathcal{M}_0, \mathcal{M}_1 \in Mod(\rho^{\mathcal{K}'_T}(T))$, $k_\varphi \leq k'_\varphi$ with $\varphi \in T$, $k_\varphi \in \mathcal{K}_T$ and $k'_\varphi \in \mathcal{K}'_T$). As the sequence is strictly decreasing for $\preceq_T$, $\mathcal{M}_0 {\not \preceq}_T  \mathcal{M}_1$. This means, there exists $\mathcal{K}'_T$ such that $\mathcal{M}_1 \in Mod(\rho^{\mathcal{K}'_T}(T))$ and $\mathcal{M}_0 {\not \in} Mod(\rho^{\mathcal{K}'_T}(T))$. By extensivity of relaxations, there exists $k_\varphi \in \mathcal{K}$ such that $k'_\varphi < k_\varphi$ with $k'_\varphi \in \mathcal{K}'_T$ and for every $k_\psi \neq k_\varphi \in \mathcal{K}$, $k'_\psi \leq k_\psi$. Let us set $\mathcal{K}_0 = \mathcal{K}'_T$, and let us write $\mathcal{K} > \mathcal{K}_0$. In the same way, we have that $\mathcal{M}_2 \prec_T \mathcal{M}_1$ but $\mathcal{M}_1 {\not \preceq}_T \mathcal{M}_2$. Hence, there exists $\mathcal{K}'_T$ such that $\mathcal{M}_2 \in Mod(\rho^{\mathcal{K}'_T}(T))$ and $\mathcal{M}_1 {\not \in} Mod(\rho^{\mathcal{K}'_T}(T))$. Let us set $\mathcal{K}_1 = \mathcal{K}'_T$. By extensivity of relaxations, we can then deduce that $\mathcal{K}_0 > \mathcal{K}_1$. By iterating this process on the sequence $(\mathcal{M}_i)_{i \in \mathbb{N}}$, we obtain an infinite decreasing sequence $(\mathcal{K}_i)_{i \in \mathbb{N}}$ which is not possible,and then is a contradiction \Marc{C'est ici o\`u ma conclusion n'est possible que si $T$ est de cardinalit\'e finie} . As $T'$ is consistent, $Mod(T') \setminus Triv$ is not empty whence we can deduce that $Min(Mod(T') \setminus Triv,\preceq_T) \neq \emptyset$.

\Isa{Discussion avec Jamal : il faut vraisemblablement supposer en plus que $\rho$ est ind\'ependant de la syntaxe pour avoir la 3e condition des FA, et donc G4.}

\Isa{Il faut aussi montrer la premi\`ere condition suppl\'entaire (Min non vide si $T'$ consistent).}

It remains to show that $Mod(T \circ T') = Min(Mod(T') \setminus Triv,\preceq_T)$. 

%To simplify the proof, we suppose that $T \circ T' = \rho^\mathcal{K}(T) \cup T'$ (i.e. if $T = T_1 \coprod T_2$, then  $T_2 = \emptyset$), the more general case where $T_2 \neq \emptyset$ being easily obtained from this more simple case.


\begin{itemize}
\item Let us first show that $Mod(T \circ T') \subseteq Min(Mod(T') \setminus Triv,\preceq_T)$. Let $\mathcal{M} \in Mod(T \circ T')$. By definition of $\circ$, there exists $\mathcal{K} = \{k_\varphi \mid \varphi \in T\}$ such that $\mathcal{M} \in Mod(\rho^\mathcal{K}(T) \cup T')$, and for every $\mathcal{K}' = \{k'_\varphi \mid \varphi \in T\}$ such that there exists $\varphi \in T$ with $k'_\varphi < k_\varphi$, $\rho^{\mathcal{K}'}(T) \cup T'$ is inconsistent. Therefore, for every $\mathcal{M}' \in Mod(\rho^{\mathcal{K}''}(T) \cup T')$, we have that $\forall \varphi \in T, k''_\varphi \geq k_\varphi$. By extensivity, we can deduce that $\mathcal{M} \preceq_T \mathcal{M}'$, whence we can conclude that $\mathcal{M} \in Min(Mod(T') \setminus Triv,\preceq_T)$. \Isa{Faut-il commenter le fait qu'on a bien $\mathcal{M} \notin Triv$ ?}
\item $Min(Mod(T') \setminus Triv,\preceq_T) \subseteq Mod(T \circ T')$. Let $\mathcal{M} \in Min(Mod(T') \setminus Triv,\preceq_T)$. By definition of $\circ$, there exists a set $\mathcal{K}$ wth minimal values $k_\varphi$ such that $\rho^\mathcal{K}(T) \cup T'$ is consistent and $T \circ T' = \rho^\mathcal{K}(T) \cup T'$. As $\mathcal{M} \in  Min(Mod(T') \setminus Triv,\preceq_T)$, this means that for every $\mathcal{M}' \in \rho^\mathcal{K}(T)$ we have $\mathcal{M} \preceq_T \mathcal{M}'$, and then $\mathcal{M} \in \rho^\mathcal{K}(T)$, whence we can conclude that $\mathcal{M} \in Mod(T \circ T')$.  
\end{itemize}
\end{proof}

%\begin{corollary}
%The revision $\circ$ of Definition~\ref{revision based in relaxation} satisfies (G1)-(G5). \Isa{Du coup il faudra pr\'eciser avec quelles hypoth\`eses sur $\rho$.}
%\end{corollary}

%\begin{proof}
%This directly follows from Theorems~\ref{correspondence agm and orders} and~\ref{orders and relaxation}
%\end{proof}
